3D CO-TALIF distribution above a micro cavity discharge: A systematic approach for plasma catalysis

We investigate a micro cavity plasma array (MCPA) reactor operated at atmospheric pressure, offering excellent diagnostic accessibility and flexible opportunities for catalyst integration. Dissociation processes, such as $\mathrm{CO}$ production from $\mathrm{CO}_{2}$ diluted in helium, are studied. The diagnostic setup, combining TALIF with an ICCD camera, enables three-dimensional spatially resolved measurements of $\mathrm{CO}$ number densities above the $\mathrm{CO}$-generating discharges. The measured distributions are compared to a basic three-dimensional diffusion model, showing good agreement and revealing the dominant transport mechanisms. Flow variation studies indicate that the gas flow inside the reactor follows a laminar, Poiseuille-like profile, while the transport behavior is consistent with literature values for the diffusion coefficient of $\mathrm{CO}$, further validating the model. The high estimated local dissociation within the MCPA discharges (about $40\%$) results in saturation of $\mathrm{CO}$ production under increasing voltage. Combined with complementary diagnostics developed for this discharge, including measurements of surface charges, electric fields, and atomic oxygen, this approach provides a suitable platform for systematic studies of plasma catalyst interactions.

==> comments.tex <==


